Faithfulness of the 2-Braid Group via Zigzag Algebra in Type B

We show that certain category of bimodules over a finite dimensional quiver algebra known as type B zigzag algebra is a quotient category of the category of type B Soergel bimodules. This leads to an alternate proof of Rouquier's conjecture on the faithfulness of the 2-braid groups for type B.

==> bibB2.tex <==
@article {KT07,
    AUTHOR = {Khovanov, Mikhail and Thomas, Richard},
     TITLE = {Braid cobordisms, triangulated categories, and flag varieties},
   JOURNAL = {Homology Homotopy Appl.},
  FJOURNAL = {Homology, Homotopy and Applications},
    VOLUME = {9},
      YEAR = {2007},
    NUMBER = {2},
     PAGES = {19--94},
      ISSN = {1532-0073},
   MRCLASS = {18E30 (14F05 18D10 20F36)},
  MRNUMBER = {2366943},
MRREVIEWER = {Matthias K\"{u}nzer},
       URL = {http://projecteuclid.org/euclid.hha/1201127331},
}

@article {Soergel92,
    AUTHOR = {Soergel, Wolfgang},
     TITLE = {The combinatorics of {H}arish-{C}handra bimodules},
   JOURNAL = {J. Reine Angew. Math.},
  FJOURNAL = {Journal f\"{u}r die Reine und Angewandte Mathematik. [Crelle's
              Journal]},
    VOLUME = {429},
      YEAR = {1992},
     PAGES = {49--74},
      ISSN = {0075-4102},
   MRCLASS = {17B10 (22E47)},
  MRNUMBER = {1173115},
MRREVIEWER = {Ronald S. Irving},
       DOI = {10.1515/crll.1992.429.49},
       URL = {https://doi.org/10.1515/crll.1992.429.49},
}

@article {SeiTho,
    AUTHOR = {Seidel, Paul and Thomas, Richard},
     TITLE = {Braid group actions on derived categories of coherent sheaves},
   JOURNAL = {Duke Math. J.},
  FJOURNAL = {Duke Mathematical Journal},
    VOLUME = {108},
      YEAR = {2001},
    NUMBER = {1},
     PAGES = {37--108},
      ISSN = {0012-7094},
   MRCLASS = {14F05 (14J32 18E30 20F36 53D40)},
  MRNUMBER = {1831820},
MRREVIEWER = {Mikhail G. Khovanov},
       DOI = {10.1215/S0012-7094-01-10812-0},
       URL = {https://doi.org/10.1215/S0012-7094-01-10812-0},
}

@article {Bige_Burau,
    AUTHOR = {Bigelow, Stephen},
     TITLE = {The {B}urau representation is not faithful for {$n=5$}},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry and Topology},
    VOLUME = {3},
      YEAR = {1999},
     PAGES = {397--404},
      ISSN = {1465-3060},
   MRCLASS = {20F36},
  MRNUMBER = {1725480},
MRREVIEWER = {Darren D. Long},
       DOI = {10.2140/gt.1999.3.397},
       URL = {https://doi.org/10.2140/gt.1999.3.397},
}


@article {Arn,
    AUTHOR = {Arnol\cprime{d}, V. I.},
     TITLE = {Critical points of functions on a manifold with boundary, the
              simple {L}ie groups {$B_{k}$}, {$C_{k}$}, {$F_{4}$} and
              singularities of evolutes},
   JOURNAL = {Uspekhi Mat. Nauk},
  FJOURNAL = {Akademiya Nauk SSSR i Moskovskoe Matematicheskoe Obshchestvo.
              Uspekhi Matematicheskikh Nauk},
    VOLUME = {33},
      YEAR = {1978},
    NUMBER = {5(203)},
     PAGES = {91--105, 237},
      ISSN = {0042-1316},
   MRCLASS = {58C25 (14B05 14B07 32C40 58C27 58F14)},
  MRNUMBER = {511883},
  DOI = { 10.1070/RM1978v033n05ABEH002515},
MRREVIEWER = {Helmut Hamm},
}


@book {SlowFour,
    AUTHOR = {Slodowy, Peter},
     TITLE = {Four lectures on simple groups and singularities},
    SERIES = {Communications of the Mathematical Institute,
              Rijksuniversiteit Utrecht},
    VOLUME = {11},
 PUBLISHER = {Rijksuniversiteit Utrecht, Mathematical Institute, Utrecht},
      YEAR = {1980},
     PAGES = {ii+64},
   MRCLASS = {14B05 (14J17 17B20 20C30 32B30)},
  MRNUMBER = {563725},
MRREVIEWER = {I. Dolgachev},
}

@book {SlowSim,
    AUTHOR = {Slodowy, Peter},
     TITLE = {Simple singularities and simple algebraic groups},
    SERIES = {Lecture Notes in Mathematics},
    VOLUME = {815},
 PUBLISHER = {Springer, Berlin},
      YEAR = {1980},
     PAGES = {x+175},
      ISBN = {3-540-10026-1},
   MRCLASS = {14J17 (20G15 32B30)},
  MRNUMBER = {584445},
MRREVIEWER = {Jonathan M. Wahl},
}



@book {Arn2,
    AUTHOR = {Arnold, V. I. and Gusein-Zade, S. M. and Varchenko, A. N.},
     TITLE = {Singularities of differentiable maps. {V}olume 2},
    SERIES = {Modern Birkh\"{a}user Classics},
      NOTE = {Monodromy and asymptotics of integrals,
              Translated from the Russian by Hugh Porteous and revised by
              the authors and James Montaldi,
              Reprint of the 1988 translation},
 PUBLISHER = {Birkh\"{a}user/Springer, New York},
      YEAR = {2012},
     PAGES = {x+492},
      ISBN = {978-0-8176-8342-9},
   MRCLASS = {58K55 (32B15 32C05 32G10 32S40 58K10)},
  MRNUMBER = {2919697},
}

@book {Arn1,
    AUTHOR = {Arnold, V. I. and Goryunov, V. V. and Lyashko, O. V. and
              Vasil\cprime ev, V. A.},
     TITLE = {Singularity theory. {I}},
      NOTE = {Translated from the 1988 Russian original by A. Iacob,
              Reprint of the original English edition from the series
              Encyclopaedia of Mathematical Sciences [{{\i}t Dynamical
              systems. VI}, Encyclopaedia Math. Sci., 6, Springer, Berlin,
              1993;  MR1230637 (94b:58018)]},
 PUBLISHER = {Springer-Verlag, Berlin},
      YEAR = {1998},
     PAGES = {iv+245},
      ISBN = {3-540-63711-7},
   MRCLASS = {58C27 (32Sxx)},
  MRNUMBER = {1660090},
       DOI = {10.1007/978-3-642-58009-3},
       URL = {https://doi.org/10.1007/978-3-642-58009-3},
}



@book {Sei,
    AUTHOR = {Seidel, Paul},
     TITLE = {Fukaya categories and {P}icard-{L}efschetz theory},
    SERIES = {Zurich Lectures in Advanced Mathematics},
 PUBLISHER = {European Mathematical Society (EMS), Z\"{u}rich},
      YEAR = {2008},
     PAGES = {viii+326},
      ISBN = {978-3-03719-063-0},
   MRCLASS = {53D40 (16E45 32Q65 53D12)},
  MRNUMBER = {2441780},
MRREVIEWER = {Timothy Perutz},
       DOI = {10.4171/063},
       URL = {https://doi.org/10.4171/063},
}


@article{KhoSei,
 ISSN = {08940347, 10886834},
 URL = {http://www.jstor.org/stable/827096},
 author = {Mikhail Khovanov and Paul Seidel},
 journal = {Journal of the American Mathematical Society},
 number = {1},
 pages = {203--271},
 publisher = {American Mathematical Society},
 title = {Quivers, {F}loer Cohomology, and Braid Group Actions},
 volume = {15},
 year = {2002}
}

@article{heng_nge,
      title={Curves in the disc, the type B braid group, and the type B zigzag algebra}, 
      author={Edmund Heng and Kie Seng Nge},
      year={2023},
      eprint={1911.12955},
      archivePrefix={arXiv},
      primaryClass={math.GT},
      journal = {To appear in Quantum Topology}
      
}


@misc{GTW,
    title={Categorical action of the extended braid group of affine type {A}},
    author={Agnes Gadbled and Anne-Laure Thiel and Emmanuel Wagner},
    year={2015},
    eprint={1504.07596},
    archivePrefix={arXiv},
    primaryClass={math.GT}
}

@misc{Ito,
    title={Curve diagram for {A}rtin group of type {B}},
    author={Tetsuya Ito},
    year={2013},
    eprint={1310.0546},
    archivePrefix={arXiv},
    primaryClass={math.GR}
}

@article{BH,
 ISSN = {0003486X},
 URL = {http://www.jstor.org/stable/1970830},
 author = {Joan S. Birman and Hugh M. Hilden},
 journal = {Annals of Mathematics},
 number = {3},
 pages = {424--439},
 publisher = {Annals of Mathematics},
 title = {On Isotopies of Homeomorphisms of {R}iemann Surfaces},
 volume = {97},
 year = {1973}
}



@book {ComCox,
    AUTHOR = {Bj\"{o}rner, Anders and Brenti, Francesco},
     TITLE = {Combinatorics of {C}oxeter groups},
    SERIES = {Graduate Texts in Mathematics},
    VOLUME = {231},
 PUBLISHER = {Springer, New York},
      YEAR = {2005},
     PAGES = {xiv+363},
      ISBN = {978-3540-442387; 3-540-44238-3},
   MRCLASS = {05-01 (05E15 20F55)},
  MRNUMBER = {2133266},
MRREVIEWER = {Jian-yi Shi},
}




@book {BraidGroups,
    AUTHOR = {Kassel, Christian and Turaev, Vladimir},
     TITLE = {Braid groups},
    SERIES = {Graduate Texts in Mathematics},
    VOLUME = {247},
      NOTE = {With the graphical assistance of Olivier Dodane},
 PUBLISHER = {Springer, New York},
      YEAR = {2008},
     PAGES = {xii+340},
      ISBN = {978-0-387-33841-5},
   MRCLASS = {20F36 (20C08 20F10 20F60 20M05 55R80 57M25 57M50)},
  MRNUMBER = {2435235},
MRREVIEWER = {Stephen P. Humphries},
       DOI = {10.1007/978-0-387-68548-9},
       URL = {https://doi.org/10.1007/978-0-387-68548-9},
}


@book{PrimerMCG,
 ISBN = {9780691147949},
 URL = {http://www.jstor.org/stable/j.ctt7rkjw},
 abstract = {The study of the mapping class group Mod(S) is a classical topic that is experiencing a renaissance. It lies at the juncture of geometry, topology, and group theory. This book explains as many important theorems, examples, and techniques as possible, quickly and directly, while at the same time giving full details and keeping the text nearly self-contained. The book is suitable for graduate students.A Primer on Mapping Class Groupsbegins by explaining the main group-theoretical properties of Mod(S), from finite generation by Dehn twists and low-dimensional homology to the Dehn-Nielsen-Baer theorem. Along the way, central objects and tools are introduced, such as the Birman exact sequence, the complex of curves, the braid group, the symplectic representation, and the Torelli group. The book then introduces Teichmüller space and its geometry, and uses the action of Mod(S) on it to prove the Nielsen-Thurston classification of surface homeomorphisms. Topics include the topology of the moduli space of Riemann surfaces, the connection with surface bundles, pseudo-Anosov theory, and Thurston's approach to the classification.},
 author = {Benson Farb and Dan Margalit},
 publisher = {Princeton University Press},
 title = {A Primer on Mapping Class Groups (PMS-49)},
 year = {2012}
}

@article{Piek,
author = "Piekosz, Artur",
journal = "Topol. Methods Nonlinear Anal.",
number = "2",
pages = "359--370",
publisher = "Nicolaus Copernicus University, Juliusz P. Schauder Centre for Nonlinear Studies",
title = "Basic definitions and properties of topological branched coverings",
url = "https://projecteuclid.org:443/euclid.tmna/1479265246",
volume = "8",
year = "1996"
}

@article{DR,
title = "On algebras of finite representation type",
journal = "Journal of Algebra",
volume = "33",
number = "2",
pages = "306 - 394",
year = "1975",
issn = "0021-8693",
doi = "https://doi.org/10.1016/0021-8693(75)90125-8",
url = "http://www.sciencedirect.com/science/article/pii/0021869375901258",
author = "Vlastimil Dlab and Claus Michael Ringel"
}

@ARTICLE{Green,
       author = {{Green}, R.~M.},
        title = "{Generalized {T}emperley-{L}ieb algebras and decorated tangles}",
      journal = {eprint arXiv:q-alg/971201},
     keywords = {Quantum Algebra and Topology, Mathematics - Quantum Algebra, 16B50, 05E99},
         year = "1997",
        month = "12",
          eid = {q-alg/9712018},
        pages = {q-alg/9712018},
archivePrefix = {arXiv},
       eprint = {q-alg/9712018},
 primaryClass = {math.QA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997q.alg....12018G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Article{KhoBiadj,
author="Khovanov, Mikhail",
title="Categorifications from planar diagrammatics",
journal="Japanese Journal of Mathematics",
year="2010",
month="Dec",
day="01",
volume="5",
number="2",
pages="153--181",
abstract="A diagrammatic presentation of functors and natural transformations and the virtues of biadjointness are discussed. We then review a graphical description of the category of Soergel bimodules and a diagrammatic categorification of positive halves of quantum groups. These notes are a write-up of Takagi Lectures given by the author in Hokkaido University in June 2009.",
issn="1861-3624",
doi="10.1007/s11537-010-0925-x",
url="https://doi.org/10.1007/s11537-010-0925-x"
}

@misc{LicQuef,
    title={Braid groups of type {A}{D}{E}, {G}arside monoids, and the categorified root lattice},
    author={Anthony M. Licata and Hoel Queffelec},
    year={2017},
    eprint={1703.06011},
    archivePrefix={arXiv},
    primaryClass={math.QA}
}

@misc{Rouq,
    title={Categorification of the braid groups},
    author={Raphael Rouquier},
    year={2004},
    eprint={math/0409593},
    archivePrefix={arXiv},
    primaryClass={math.RT}
}

@article{MackTubb, title={Two-color {S}oergel Calculus and Simple Transitive 2-representations}, volume={71}, DOI={10.4153/CJM-2017-061-2}, number={6}, journal={Canadian Journal of Mathematics}, publisher={Canadian Mathematical Society}, author={Mackaaij, Marco and Tubbenhauer, Daniel}, year={2019}, pages={1523–1566}}

@article{HueKho,
title = "A Category for the Adjoint Representation",
journal = "Journal of Algebra",
volume = "246",
number = "2",
pages = "514 - 542",
year = "2001",
issn = "0021-8693",
doi = "https://doi.org/10.1006/jabr.2001.8962",
url = "http://www.sciencedirect.com/science/article/pii/S0021869301989628",
author = "Ruth Stella Huerfano and Mikhail Khovanov",
keywords = "quantum groups, Dynkin diagrams, McKay correspondence, quivers, categorification",
abstract = "We construct an abelian category C and exact functors in C which on the Grothendieck group descend to the action of a simply laced quantum group in its adjoint representation. The braid group action in the adjoint representation lifts to an action in the derived category of C. The category C is the direct sum of a semisimple category and the category of modules over a certain algebra associated with a Dynkin diagram. In the second half of the paper we show how these algebras appear in the modular representation theory and in the McKay correspondence and explore their relationship with root systems"
}

@article{brav_thomas_2010, title={Braid groups and Kleinian singularities}, volume={351}, DOI={10.1007/s00208-010-0627-y}, number={4}, journal={Mathematische Annalen}, author={Brav, Christopher and Thomas, Hugh}, year={2010}, pages={1005–1017}}

@misc{LinkHom,
      title={Notes on link homology}, 
      author={Marta Asaeda and Mikhail Khovanov},
      year={2008},
      eprint={0804.1279},
      archivePrefix={arXiv},
      primaryClass={math.QA}
}

@article{rouquier_2006, title={Categorification of sl2 and braid groups}, DOI={10.1090/conm/406/07657}, journal={Trends in Representation Theory of Algebras and Related Topics Contemporary Mathematics}, author={Rouquier, Raphaël}, year={2006}, pages={137–167}}

@article {Soergel_07,
    AUTHOR = {Soergel, Wolfgang},
     TITLE = {Kazhdan-{L}usztig-{P}olynome und unzerlegbare {B}imoduln \"{u}ber
              {P}olynomringen},
   JOURNAL = {J. Inst. Math. Jussieu},
  FJOURNAL = {Journal of the Institute of Mathematics of Jussieu. JIMJ.
              Journal de l'Institut de Math\'{e}matiques de Jussieu},
    VOLUME = {6},
      YEAR = {2007},
    NUMBER = {3},
     PAGES = {501--525},
      ISSN = {1474-7480},
   MRCLASS = {20C08 (20F55)},
  MRNUMBER = {2329762},
MRREVIEWER = {Ulrich G\"{o}rtz},
       DOI = {10.1017/S1474748007000023},
       URL = {https://doi.org/10.1017/S1474748007000023},
}

@article{EW_2016, title={Soergel calculus}, volume={20}, DOI={10.1090/ert/481}, number={12}, journal={Representation Theory of the American Mathematical Society}, author={Elias, Ben and Williamson, Geordie}, year={2016}, pages={295–374}}

@mastersthesis{jensen_master,
  author       = {Lars Thorge Jensen}, 
  title        = {Categorification of Braid Groups},
  school       = {Mathematisch-Naturwissenschaftliche Fakultat Der Rheinischen Friedrich-Wilhelms-Universitat Bonn},
  year         = {2014}}
  

@article{jensen_2016, title={The 2-braid group and Garside normal form}, volume={286}, DOI={10.1007/s00209-016-1769-8}, number={1-2}, journal={Mathematische Zeitschrift}, author={Jensen, Lars Thorge}, year={2016}, pages={491–520}}

@article{crisp_1997, title={Injective maps between Artin groups}, DOI={10.1515/9783110806861.119}, journal={Geometric Group Theory Down Under}, author={Crisp, John}, year={1997}}
